Light-cone feature selection in methane hyperspectral images

Hyperspectral images (HSIs) capture detailed spectral information across numerous contiguous bands, enabling the extraction of intrinsic characteristics of scanned objects and areas. This study focuses on the application of light-cone feature selection in quantum machine learning for methane detection and localization using HSIs. The proposed method leverages quantum methods to enhance feature selection and classification accuracy. The dataset used includes HSIs collected by the AVIRIS-NG instrument captured in geographically diverse locations. In this study, we investigate the performance of support vector machine classifiers with different classic and quantum kernels. The results indicate that the quantum kernel classifier, combined with light-cone feature selection, provides in one metric, superior performance when compared to the classic techniques. It demonstrates the potential of quantum machine learning in improving the remote sensing data analysis for environmental monitoring.

==> tikz_backup.tex <==
\begin{figure*}
    \centering

\begin{quantikz}
\lstick{$\ket{0}$} & \gate[style={fill={rgb,255:red,23;green,190;blue,207},fill opacity=0.3}]{V(x_1)} & \gate[2, style={fill={rgb,255:red,23;green,190;blue,207},fill opacity=0.3}]{U(\Theta_{1,1})} &  \gate{V(x_1)} & \gate{U(\Theta_{2,1})} & \gate{V(x_1)} & \gate[2]{U(\Theta_{3,1})} & \meter{} \\
\lstick{$\ket{0}$} & \gate[style={fill={rgb,255:red,23;green,190;blue,207},fill opacity=0.3}]{V(x_2)} & \qw &  \gate[style={fill={rgb,255:red,23;green,190;blue,207},fill opacity=0.3}]{V(x_2)} & \gate[2, style={fill={rgb,255:red,23;green,190;blue,207},fill opacity=0.3}]{U(\Theta_{2,2})} & \gate{V(x_2)} & \qw & \meter{} \\
\lstick{$\ket{0}$} & \gate[style={fill={rgb,255:red,23;green,190;blue,207},fill opacity=0.3}]{V(x_3)} & \gate[2, style={fill={rgb,255:red,23;green,190;blue,207},fill opacity=0.3}]{U(\Theta_{1,2})}  & \gate[style={fill={rgb,255:red,23;green,190;blue,207},fill opacity=0.3}]{V(x_3)} & \qw & \gate[style={fill={rgb,255:red,23;green,190;blue,207},fill opacity=0.3}]{V(x_3)} & \gate[2, style={fill={rgb,255:red,23;green,190;blue,207},fill opacity=0.3}]{U(\Theta_{3,2})} & \meter{} \\
\lstick{$\ket{0}$} & \gate[style={fill={rgb,255:red,23;green,190;blue,207},fill opacity=0.3}]{V(x_4)} &  \qw      & \gate[style={fill={rgb,255:red,23;green,190;blue,207},fill opacity=0.3}]{V(x_4)} & \gate[2, style={fill={rgb,255:red,23;green,190;blue,207},fill opacity=0.3}]{U(\Theta_{2,3})}  &  \gate[style={fill={rgb,255:red,23;green,190;blue,207},fill opacity=0.3}]{V(x_4)} & \qw & \meter[style={fill={rgb,255:red,23;green,190;blue,207},fill opacity=0.3}]{} \\
\lstick{$\ket{0}$} & \gate[style={fill={rgb,255:red,23;green,190;blue,207},fill opacity=0.3}]{V(x_5)} & \gate[2, style={fill={rgb,255:red,23;green,190;blue,207},fill opacity=0.3}]{U(\Theta_{1,3})}  &  \gate[style={fill={rgb,255:red,23;green,190;blue,207},fill opacity=0.3}]{V(x_5)} & \qw & \gate{V(x_5)} & \gate[2]{U(\Theta_{3,3})}  & \meter{} \\
\lstick{$\ket{0}$} & \gate[style={fill={rgb,255:red,23;green,190;blue,207},fill opacity=0.3}]{V(x_6)} & \qw      & \gate{V(x_6)} & \gate{U(\Theta_{2,1})} & \gate{V(x_6)} & \qw      & \meter{} \\
\end{quantikz}

    \caption{Schematic representation of the light-cone feature selection circuit with $n=6$, $L=3$. It consists of the alternating layers of one-qubit and two-qubit gates. One qubit gates, $V(x_i)$ are responsible for the re-uploading of the $i^{th}$ feature of the data point $x$. Two-qubit blocks $U(\Theta_{k,l})$ are responsible for the information propagation of the features throughout the qubits. Each of the qubit is measured at the end and gives a rise to the local, projected kernel. With light-blue we highlight the measurement of the fourth qubit and its light-cone.
    The weights for the importance score for the highlighted local kernel are $w_{\lambda_4} (x_1) = w_{\lambda_4} (x_6) = 1,\ w_{\lambda_4}(x_2) = w_{\lambda_4} (x_5) = 2,\ w_{\lambda_4} (x_3) = w_{\lambda_4} (x_4) = 3$.}
    \label{fig:enter-label}
\end{figure*}

